Point-wise Stability of Reaction Diffusion Fronts

Using pointwise semigroup techniques, we establish sharp rates of decay in space and time of a perturbed reaction diffusion front to its time-asymptotic limit. This recovers results of Sattinger, Henry and others of time-exponential convergence in weighted $L^p$ and Sobolev norms, while capturing the new feature of spatial diffusion at Gaussian rate. Novel features of the argument are a point-wise Green function decomposition reconciling spectral decomposition and short-time Nash-Aronson estimates and an instantaneous tracking scheme similar to that used in the study of stability of viscous shock waves.

==> rsemacros.tex <==
%%
%% This is file `rsemacros.tex'
%% Royal Society of Edinburgh Macros File for Series A Journal
%%
%% Copyright 1998 T&T Productions Ltd
%%
%% Developed by Jonathan Wainwright
%%
%% 19.2.99 `\meas' macro defined
%%
\def\fileversion{v1.02}
\def\filedate{1999/02/19}
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%    CONTENTS            %
% ====================== %
% 1. EDITING MACROS      %
% 2. UNITS               %
% 3. MATHS MACROS        %
% 4. GREEK MACROS        %
% 5. FIGURES             %
% 6. SUBEQUATION         %
%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%
% EDITING MACROS %
%%%%%%%%%%%%%%%%%%

% \tit  Abbreviation for `\textit'
\newcommand{\tit}[1]{\textit{#1}}

% \tbf  Abbreviation for `\textbf'
\newcommand{\tbf}[1]{\textbf{#1}}

% \tsc  Abbreviation for `\textsc'
\newcommand{\tsc}[1]{\textsc{#1}}

% \mrm  Abbreviation for `\mathrm'
\newcommand{\mrm}[1]{\mathrm{#1}}

% \present Macro for `present address' for use in \author
\newcommand{\present}[1]{\footnote{Present address: #1}}

% \permanent Macro for `permanent address' for use in \author
\newcommand{\permanent}[1]{\footnote{Permanent address: #1}}

% \email Macro for `email address' for use in \affiliation
\newcommand{\email}[1]{{\upshape(\texttt{#1})}}
\newcommand{\twoemails}[2]{{\upshape(\texttt{#1}; \texttt{#2})}}

% \ca   Use only before a number; otherwise use `about',
%       `approximately', etc. - \ca10
%
\newcommand{\ca}{\textit{ca}.\kern1.66pt}

% \et   Omits extra full stop after et al. if at end of sentence,
%       and uses xspace to avoid any unwanted space
%
\makeatletter
\newcommand{\@etalstop}{\ifx\@let@token.%
                          \else.%
                        \fi\xspace}
\newcommand{\etalstop}{\futurelet\@let@token\@etalstop}
\newcommand{\et}{\textit{et al}\etalstop}
\makeatother

% \OK   OK query - prints `OK?' in the margin
%
\newcommand{\OK}[1]{\protect\smash{\underline{#1}}\marginpar{\underline{OK?}}}

% \query   Extended query - prints more detailed query in margin
%
\newcommand{\query}[2]{\protect\smash{\underline{#1}}%
  \marginpar{\small\raggedright#2}}
\newcommand{\gquery}[2]{\query{#1}{#2-\hbox{\raisebox{0.15mm}%
  {$\bigcirc$}\hspace{-2.9mm}\footnotesize{G}}}}

% \mpar   Marginal query for use without underlining text.
%
\newcommand{\mpar}[1]{\marginpar{\small\raggedright#1}}
\newcommand{\empar}[1]{\mpar{\small\raggedright\ \\[-12mm]#1}}

% \press      (In the press.)
% \submitted  (Submitted.)
% \prep       (In preparation.)
% \publ        Publisher?
% \notcited   Not cited in text!
% \details    Details?
% \notinrefs  Not in references!
% \allauthors Provide all authors!
%
\newcommand{\press}{\underline{(In the press.)}\marginpar{\small Details?}}
\newcommand{\submitted}{\underline{(Submitted.)}\marginpar{\small Details?}}
\newcommand{\prep}{\underline{(In preparation.)}\marginpar{\small Details?}}
\newcommand{\publ}{\underline{Publisher.}\marginpar{\small Publisher?}}
\newcommand{\notcited}[1]{\query{#1}{\small Not cited in text!}}
\newcommand{\notinrefs}[1]{\query{#1}{\small Not in References!}}
\newcommand{\allauthors}{\query{\et}{\small Please provide all authors!}}
\newcommand{\details}{\mpar{\small Details?}}
\newcommand{\initials}{\underline{X. X. X.}\marginpar{\small Initials?}}

% \registered   For use after programs such as Adobe Illustrator
%
\newcommand{\registered}{${}^{\bigcirc\hskip-6.4pt\mbox{\tiny R}}$}

% \sect   Section symbol for use only with a section number
%
\newcommand{\sect}{{\usefont{OMS}{cmsy}{m}{n}\S\,}}

% \ns   Natural spacing using \letterspace for use in author names
%
\newcommand{\ns}[1]{\letterspace to 1.15\naturalwidth{#1}}

% \ui   Upright item label
%
\newcommand{\ui}[1]{\item[{\upshape(#1)}]}
\newcommand{\uinp}[1]{\item[{\upshape#1}]}

% \bye  End document
%
\newcommand{\bye}{\label{lastpage}\end{document}}

% \ack  Acknowledgments
%
\newcommand{\ack}{\section*{Acknowledgments}}

% \Issued  For final line
%
\newcommand{\Issued}[1]{\medbreak\centering\footnotesize(\textit{Issued #1})}

\newcommand{\blankoddpage}{\newpage{\thispagestyle{blank}\phantom{blank}}}
\newcommand{\blankevenpage}{\newpage{\thispagestyle{blank}}\cleardoublepage}

% Errata macros
%
\newcommand{\errtitle}[1]{\section*{#1}}
\newcommand{\errauthor}[1]{\centerline{\textsc{By #1}}\bigskip}
\newcommand{\errrefpa}[3]{\centerline{\textit{Proc. R. Soc. Lond.}
A\,\textbf{#1}, #2 (#3)}\bigskip}
\newcommand{\errrefta}[3]{\centerline{\textit{Phil. Trans. R. Soc. Lond.}
A\,\textbf{#1}, #2 (#3)}\bigskip}

%%%%%%%%%%%
%  UNITS  %
%%%%%%%%%%%

% \3   Fixed unbreakable space separating numbers and their units
%      e.g. 5\3cm (no need to group the unit)
%
\newcommand{\3}{\kern2.5pt}

% \C   Degrees Celcius
%      Use in text or math, no need to mbox or add space
%
\newcommand{\C}[1]{\ensuremath{{}^\circ}\textrm{C}\xspace#1}

% \upmu   Upright mu for `micro-' prefix
%
\newcommand{\upmu}[1]{\Pisymbol{psy}{109}#1}

%%%%%%%%%%%%%%%%
% MATHS MACROS %
%%%%%%%%%%%%%%%%

\newcommand{\nn}{\nonumber}
\newcommand{\RE}{R\kern-.667pte}  % Reynolds number
\newcommand{\PR}{P\kern-.667ptr}  % Prandtl number
\newcommand{\NU}{N\kern-.667ptu}  % Nusselt number

\newcommand{\dsty}{\displaystyle}
\newcommand{\ssty}{\scriptstyle}

\newcommand{\link}[1]{\quad\text{#1}\quad} % Linking roman text

% Use AMS binary relations in preference to standard LaTeX symbols
\let\le\leqslant
\let\leq\leqslant
\let\ge\geqslant
\let\geq\geqslant

% `Greater than less than' relation
\newcommand{\gtlt}{\stackrel{\raisebox{2pt}{$\scriptstyle >$}}%
  {\smash{\scriptstyle <}}}

\newcommand{\rd}{\mathrm{d}}            % Roman d for differential
\newcommand{\re}{\mathrm{e}}            % Roman e for exponential
\newcommand{\ri}{\mathrm{i}}            % Roman i for imaginary number
\newcommand{\cc}{\mathrm{c.c.}}         % Abbreviation for `complex conjugate'
\newcommand{\const}{\mathrm{const.}}    % Abbreviation for `constant'

\newcommand{\triup}{\vartriangle}
\newcommand{\tridown}{\triangledown}
\newcommand{\triright}{\vartriangleright}
\newcommand{\trileft}{\vartriangleleft}
\newcommand{\btriup}{\blacktriangle}
\newcommand{\btridown}{\blacktriangledown}
\newcommand{\btriright}{\blacktriangleright}
\newcommand{\btrileft}{\blacktriangleleft}
\newcommand{\bsquare}{{\scriptscriptstyle\blacksquare}}
\newcommand{\blozenge}{\blacklozenge}
\newcommand{\ssquare}{{\scriptscriptstyle\square}}

\DeclareMathOperator{\Real}{Re}  % Real part
\DeclareMathOperator{\Imag}{Im}  % Imaginary part
\DeclareMathOperator{\diag}{diag}         % Diagonal
\DeclareMathOperator{\Int}{Int}           % Integer
\DeclareMathOperator{\Mod}{mod}           % Modulus (de-spaced)
\DeclareMathOperator{\sgn}{sgn}           % Sign
\DeclareMathOperator{\res}{res}           % Residue
\DeclareMathOperator{\Res}{Res}           % Residue
\DeclareMathOperator{\mes}{mes}           % Measure
\DeclareMathOperator{\meas}{meas}         % Measure
\DeclareMathOperator{\erf}{erf}           % Error function
\DeclareMathOperator{\erfc}{erfc}         % Complementary error function
\DeclareMathOperator{\rank}{rank}         % Rank
\DeclareMathOperator{\tr}{tr}             % Trace
\DeclareMathOperator{\Tr}{Tr}             % Trace
\DeclareMathOperator{\Ai}{Ai}             % Airy function
\DeclareMathOperator{\Bi}{Bi}             % Airy function
\DeclareMathOperator{\Ei}{Ei}             %
\DeclareMathOperator{\curl}{curl}         % Curl
\DeclareMathOperator{\grad}{grad}         % Grad
\DeclareMathOperator{\inc}{inc}           % Inc
\DeclareMathOperator{\Hess}{Hess}         % Hessian
\DeclareMathOperator{\arccot}{arccot}     % Inverse cotangent
\DeclareMathOperator{\arcsec}{arcsec}     % Inverse secant
\DeclareMathOperator{\arccosec}{arccosec} % Inverse cosecant
\DeclareMathOperator{\cosec}{cosec}       % Cosecant
\DeclareMathOperator{\sech}{sech}         % Hyperbolic secant
\DeclareMathOperator{\cosech}{cosech}     % Hyperbolic cosecant
\DeclareMathOperator{\arcsinh}{arsinh}    % Inverse hyperbolic sine
\DeclareMathOperator{\arcosh}{arcosh}     % Inverse hyperbolic cosine
\DeclareMathOperator{\artanh}{artanh}     % Inverse hyperbolic tangent
\DeclareMathOperator{\arcoth}{arcoth}     % Inverse hyperbolic cotangent
\DeclareMathOperator{\arsech}{arsech}     % Inverse hyperbolic secant
\DeclareMathOperator{\arcosech}{arcosech} % Inverse hyperbolic cosecant
\DeclareMathOperator{\sn}{sn}             % Jacobian elliptic sinus
\DeclareMathOperator{\cn}{cn}             % Jacobian elliptic cosinus
\DeclareMathOperator{\dn}{dn}             % elliptic functions
\DeclareMathOperator{\supp}{supp}         %
\DeclareMathOperator{\dist}{dist}         %
\DeclareMathOperator{\adj}{adj}           % adjoint
\DeclareMathOperator{\Div}{div}           % divergence
\DeclareMathOperator{\Span}{span}         % span

\newcommand{\dint}{\int\kern-5pt\int}

\newcommand{\qq}{\qquad}

\newcommand{\smfr}[2]{{\textstyle\frac{#1}{#2}}}         % Small fraction
\newcommand{\mdfr}[2]{\hbox{\small$\dsty\frac{#1}{#2}$}}   % Medium fraction

% To display maths inline with a short piece of text left justified
%
\newcommand{\InlineDisplay}[2]{\smallskip\noindent\hbox to \hsize{#1\hfill%
 \begin{math}#2\end{math}\hfill\phantom{#1}}}

% `Frown' accent (upside down \breve, almost!)
%
\newcommand{\frownaccent}[1]{\mathaccent"317F{#1}}

% Bold zero and one
\newcommand{\bzero}{\bm{0}}
\newcommand{\bone}{\bm{1}}
% Phantom zero for use in tables
\newcommand{\0}{\phantom{0}}
% Multicolumn abbreviation
\newcommand{\mc}{\multicolumn}
% Overbrace for use in tables
\newcommand{\ob}[2]{\mc{#1}{c}{$\overbrace{\hspace{#2mm}}$}}
% Smashed vertical brace
\newcommand{\vbrace}[1]{\smash{\left\{ \phantom{\rule{0.1mm}{#1mm}} \right.}}
% Left shift 1st line of an aligned structure
\newcommand{\leftshift}[1]{\hspace{#1mm}&\hspace{-#1mm}}

%%%%%%%%%%%%%%%%
% GREEK MACROS %
%%%%%%%%%%%%%%%%

% Sloping Greek caps
\newcommand{\sDe}{\varDelta}
\newcommand{\sLa}{\varLambda}
\newcommand{\sOm}{\varOmega}
\newcommand{\sSi}{\varSigma}
\newcommand{\sTh}{\varTheta}
\newcommand{\sPh}{\varPhi}
\newcommand{\sPs}{\varPsi}
\newcommand{\sPi}{\varPi}
\newcommand{\sGa}{\varGamma}
\newcommand{\sUp}{\varUpsilon}
\newcommand{\sXi}{\varXi}

% Bold Greek lowercase

\DeclareBoldMathCommand\bal{\alpha}
\DeclareBoldMathCommand\bbe{\beta}
\DeclareBoldMathCommand\bga{\gamma}
\DeclareBoldMathCommand\bde{\delta}
\DeclareBoldMathCommand\bep{\epsilon}
\DeclareBoldMathCommand\bve{\varepsilon}
\DeclareBoldMathCommand\bze{\zeta}
\DeclareBoldMathCommand\bet{\eta}
\DeclareBoldMathCommand\bth{\theta}
\DeclareBoldMathCommand\bio{\iota}
\DeclareBoldMathCommand\bka{\kappa}
\DeclareBoldMathCommand\bla{\lambda}
\DeclareBoldMathCommand\bmu{\mu}
\DeclareBoldMathCommand\bnu{\nu}
\DeclareBoldMathCommand\bxi{\xi}
\DeclareBoldMathCommand\bpi{\pi}
\DeclareBoldMathCommand\brh{\rho}
\DeclareBoldMathCommand\bsi{\sigma}
\DeclareBoldMathCommand\bta{\tau}
\DeclareBoldMathCommand\bup{\upsilon}
\DeclareBoldMathCommand\bph{\phi}
\DeclareBoldMathCommand\bvp{\varphi}
\DeclareBoldMathCommand\bch{\chi}
\DeclareBoldMathCommand\bps{\psi}
\DeclareBoldMathCommand\bom{\omega}

% Bold Greek caps

\DeclareBoldMathCommand\bDe{\varDelta}
\DeclareBoldMathCommand\bLa{\varLambda}
\DeclareBoldMathCommand\bOm{\varOmega}
\DeclareBoldMathCommand\bSi{\varSigma}
\DeclareBoldMathCommand\bTh{\varTheta}
\DeclareBoldMathCommand\bPh{\varPhi}
\DeclareBoldMathCommand\bPs{\varPsi}
\DeclareBoldMathCommand\bPi{\varPi}
\DeclareBoldMathCommand\bGa{\varGamma}
\DeclareBoldMathCommand\bUp{\varUpsilon}
\DeclareBoldMathCommand\bXi{\varXi}

% Greek caps (\Pi, \Xi, \Psi, \Phi not defined)
\newcommand{\De}{\Delta}
\newcommand{\La}{\Lambda}
\newcommand{\Om}{\Omega}
\newcommand{\Si}{\Sigma}
\newcommand{\Th}{\Theta}
\newcommand{\Ga}{\Gamma}
\newcommand{\Up}{\Upsilon}

%%%%%%%%%%%
% FIGURES %
%%%%%%%%%%%

\newcommand{\cfg}[1]{\centerline{\epsfig{file=#1.ps}}}
\newcommand{\cfig}[2]{\centerline{\epsfig{file=#1.ps,width=#2mm}}}
\newcommand{\cefg}[1]{\centerline{\epsfig{file=#1.eps}}}
\newcommand{\cefig}[2]{\centerline{\epsfig{file=#1.eps,width=#2mm}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SUBEQUATION ENVIRONMENT %
%%%%%%%%%%%%%%%%%%%%%%%%%%%

% SUBEQN redefines SUBEQUATIONS to give italic lower case counters

\newenvironment{subeqns}{\begin{subequations}%
  \renewcommand{\theequation}{\theparentequation\,$\alph{equation}$}}%
  {\end{subequations}}

\multlinegap0pt % Removes indent

\endinput
%%
%% End of file `rsemacros.tex'.

